KDA+: Understanding and Mitigating Recurrent State Instability

Linear attention offers an efficient solution for long-sequence modeling via linear complexity and fixed-size recurrent states. Gated DeltaNet-2 (GDN-2) introduces independent channel-wise control over erasure and writing, enhancing state-update expressiveness and in-context retrieval, yet it suffers from training failures during long-context training. We trace these failures to the asymmetry between reading and modification directions during erasure, which yields non-normal erase operators whose directional gains accumulate across tokens, triggering exponential state growth even without new writes. To resolve this, we draw on the symmetric delta update of Kimi Delta Attention (KDA) to develop KDA+, which introduces independent channel-wise erase and write gates while preserving non-expansive state propagation and uses decay-regulated residual writing to preserve flexibility. Theoretically, we establish an $O(\sqrt{T})$ upper bound on recurrent state growth while retaining chunkwise parallel computation. Experiments on 1.6B parameter models show that KDA+ achieves stable training alongside improved long-context retrieval. Compared to GDN-2, it boosts the 128K average RULER score by 6.80 points in the recurrent setting and average accuracy across nine downstream tasks by 0.62 points in the hybrid setting.

==> intro_backup.tex <==
The growing demand for long-context understanding and extended generation~\cite{sun2025efficient,zhang2026survey} has made efficient sequence modeling an increasingly important challenge for large language models. 
While standard softmax attention provides direct access to the entire context, its quadratic computational complexity and growing key--value cache impose substantial computational and memory overheads as sequence length increases~\cite{llama2023llama}. 
To address these computational and memory bottlenecks, linear attention~\cite{katharopoulos2020transformers,retnet} has emerged as an efficient alternative that compresses historical information into a fixed-size recurrent state, thereby enabling linear-time sequence processing and constant memory during autoregressive decoding. Building on this approach, recent advances in gating mechanisms and delta-rule-based updates~\cite{gla,GDN,yang2024parallelizing} have substantially enhanced the expressiveness of recurrent memory, enabling more fine-grained control over information retention and modification. 

Gated DeltaNet-2 (GDN-2)~\cite{GDN2} further advances this line of work by replacing the shared scalar update gate in GDN~\cite{GDN} and KDA~\cite{kda} with independent vector-valued erase and write gates. This decoupling enables finer-grained control over which memory components are erased and how new information is incorporated. 
Beyond improving update flexibility, this design also fundamentally alters the geometry of memory propagation by allowing the directions used for memory retrieval and modification to diverge.
Consequently, as information propagates through long sequences, each stored contribution undergoes a composition of input-dependent transformations, making the stability of these transformations critical to reliable long-term memory retention~\cite{tiezzi2025state}.

However, our experiments reveal that the increased flexibility of GDN-2 comes at the cost of potential instability in recurrent state propagation, particularly over long sequences. At a context length of 64K, we observe numerical failures across both pretraining and post-training settings, affecting purely linear as well as hybrid GDN-2 architectures. More importantly, numerical failures represent only the most visible manifestation of a broader issue: even in runs that complete training with finite losses, individual entries of the recurrent state can exceed \(10^{36}\), indicating substantial internal state amplification. In runs that eventually diverge, the training loss often provides little indication of the impending numerical breakdown. These observations highlight a fundamental limitation of loss-based monitoring and motivate a closer investigation of the underlying recurrent state dynamics that govern memory propagation over long sequences.   
% \zxc{to be polished}

Our analysis shows that existing memory in GDN-2 can grow exponentially even after new writes cease. This growth can arise from the asymmetric coupling of the erase gate and key, which misaligns the directions used to read and modify the state. The resulting non-normal erasure operator can amplify certain state directions despite having eigenvalues within the unit disk. When directions amplified by earlier transitions align with the expanding directions of subsequent transitions, these gains can accumulate across the sequence and overcome decay. Diagnostics of actual training trajectories reveal corresponding cumulative amplification, connecting this mechanism to the observed state growth and numerical failures.


These findings motivate \model, which controls memory amplification through symmetric erasure while retaining vector-valued gating. Distributing the erase gate symmetrically across the two key factors aligns the reading and correction directions, ensuring non-expansive propagation under the standard key normalization and gate constraints. To complement the resulting gated write, we introduce a residual writing path whose amplitude is regulated by decay. This design supports additional writing in channels where the erase gate is small while controlling the energy introduced by the residual. The update retains an input-dependent affine structure compatible with chunk-wise parallel computation.

Our evaluation examines whether this stabilization improves training reliability while preserving the modeling benefits of flexible memory updates. We compare stabilization strategies across pretraining and post-training settings, assessing recurrent-state behavior, language modeling quality, long-context retrieval, and computational efficiency. 

In summary, our contributions lie in the following aspects:

==> table/ruler_small.tex <==

\begin{table*}[t]
\centering
\caption{RULER results on the four-task retrieval subset.
Scores are percentages; higher is better.
S1, S2, S3 and MK1 denote
\texttt{niah\_single\_1},
\texttt{niah\_single\_2},
\texttt{niah\_single\_3} and
\texttt{niah\_multikey\_1}, respectively.
Bold and underlined values indicate the best and second-best results
within each setting, respectively.
Ties are determined at the displayed precision.}
\label{tab:ruler_wide}

\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.25}
\fontsize{8}{9.6}\selectfont

\begin{tabularx}{\textwidth}{
    @{}p{18mm}
    >{\centering\arraybackslash}p{11mm}
    *{15}{>{\centering\arraybackslash}X}@{}
}
\toprule
\multirow{2}{*}{Method}
& \multirow{2}{*}{\makecell{\textbf{Overall}\\\textbf{Avg.}}}
& \multicolumn{5}{c}{32K}
& \multicolumn{5}{c}{64K}
& \multicolumn{5}{c}{128K} \\

\cmidrule(lr){3-7}
\cmidrule(lr){8-12}
\cmidrule(lr){13-17}
& & S1 & S2 & S3 & MK1 & \textbf{Avg.}
  & S1 & S2 & S3 & MK1 & \textbf{Avg.}
  & S1 & S2 & S3 & MK1 & \textbf{Avg.} \\
\midrule

\multicolumn{17}{@{}l}{\textit{Recurrent Setting}} \\
\addlinespace[2pt]

\quad GDN-2
& \cellcolor{black!4}18.48
& \textbf{100.00} & 2.80 & \underline{4.40} & \underline{7.40}
& \cellcolor{black!4}28.65
& 86.80 & 3.00 & 3.40 & 4.60
& \cellcolor{black!4}24.45
& 2.80 & 2.00 & 1.60 & 3.00
& \cellcolor{black!4}2.35 \\

% \quad FG-GDN
% & \cellcolor{black!4}22.22
% & \textbf{100.00} & 2.40 & 4.00 & 3.60
% & \cellcolor{black!4}27.50
% & 98.00 & 3.00 & 3.40 & 4.40
% & \cellcolor{black!4}27.20
% & 40.80 & 2.00 & \textbf{2.20} & 2.80
% & \cellcolor{black!4}11.95 \\

\quad D-Clip
& \cellcolor{black!4}16.67
& 95.00 & 3.80 & 3.00 & \textbf{9.40}
& \cellcolor{black!4}27.80
& 47.40 & 4.00 & \textbf{4.80} & \underline{6.80}
& \cellcolor{black!4}15.75
& 16.00 & \textbf{3.40} & \underline{1.80} & \textbf{4.60}
& \cellcolor{black!4}6.45 \\

\quad $\beta$-Guard
& \cellcolor{black!4}\underline{25.27}
& \underline{99.60} & \textbf{5.20} & 4.20 & \textbf{9.40}
& \cellcolor{black!4}\underline{29.60}
& 96.60 & \textbf{5.00} & \underline{4.60} & \underline{6.80}
& \cellcolor{black!4}\underline{28.25}
& \underline{64.40} & \underline{2.20}
& \textbf{2.00} & \underline{3.20}
& \cellcolor{black!4}\textbf{17.95} \\

\quad KDA
& \cellcolor{black!4}24.22
& \textbf{100.00} & 2.40 & 3.80 & 4.80
& \cellcolor{black!4}27.75
& \underline{98.20} & 2.60 & 3.20 & 4.20
& \cellcolor{black!4}27.05
& \textbf{65.00} & 1.80 & \textbf{2.00} & 2.60
& \cellcolor{black!4}\underline{17.85} \\

\midrule
\rowcolor{black!7}
\quad \textbf{Ours}
& \cellcolor{black!12}\textbf{25.43}
& \textbf{100.00} & \underline{4.00}
& \textbf{6.20} & \textbf{9.40}
& \cellcolor{black!12}\textbf{29.90}
& \textbf{99.80} & \underline{4.20}
& \textbf{4.80} & \textbf{7.60}
& \cellcolor{black!12}\textbf{29.10}
& 62.40 & 2.00 & \textbf{2.00} & 2.80
& \cellcolor{black!12}17.30 \\

\midrule
\multicolumn{17}{@{}l}{\textit{Hybrid Setting}} \\
\addlinespace[2pt]

\quad GDN-2
& \cellcolor{black!4}29.95
& 72.60 & 57.60 & 25.20 & 47.80
& \cellcolor{black!4}50.80
& 35.00 & 27.60 & 15.40 & 30.80
& \cellcolor{black!4}27.20
& 19.00 & \underline{10.40} & 2.60 & \textbf{15.40}
& \cellcolor{black!4}11.85 \\

% \quad FG-GDN
% & \cellcolor{black!4}\underline{34.23}
% & \textbf{79.20} & \textbf{68.60}
% & \underline{49.00} & 41.00
% & \cellcolor{black!4}\underline{59.45}
% & \textbf{38.40} & 27.00 & \underline{22.80} & 29.60
% & \cellcolor{black!4}29.45
% & \textbf{21.00} & 9.80 & \textbf{10.20} & 14.20
% & \cellcolor{black!4}\textbf{13.80} \\

\quad D-Clip
& \cellcolor{black!4}\textbf{36.33}
& \textbf{77.00} & \textbf{68.00}
& \textbf{49.40} & \textbf{53.60}
& \cellcolor{black!4}\textbf{62.00}
& \textbf{36.60} & \textbf{34.40}
& \textbf{28.00} & \textbf{34.20}
& \cellcolor{black!4}\textbf{33.30}
& \underline{19.80} & \textbf{11.60} & \textbf{8.00} & \textbf{15.40}
& \cellcolor{black!4}\textbf{13.70} \\

\quad $\beta$-Guard
& \cellcolor{black!4}31.88
& 74.80 & \underline{67.00} & 24.60 & 39.40
& \cellcolor{black!4}51.45
& \textbf{36.60} & \underline{33.40}
& 21.00 & \underline{32.60}
& \cellcolor{black!4}\underline{30.90}
& \textbf{20.00} & \textbf{11.60} & \underline{6.20} & \textbf{15.40}
& \cellcolor{black!4}\underline{13.30} \\

\quad KDA
& \cellcolor{black!4}24.17
& 75.80 & 38.80 & 21.20 & 34.40
& \cellcolor{black!4}42.55
& \underline{36.40} & 21.20 & 8.40 & 21.80
& \cellcolor{black!4}21.95
& 19.40 & 4.00 & 2.40 & 6.20
& \cellcolor{black!4}8.00 \\

\midrule
\rowcolor{black!7}
\quad \textbf{Ours}
& \cellcolor{black!12}\underline{33.57}
& \underline{76.40} & 62.40 & \underline{48.60} & \underline{48.80}
& \cellcolor{black!12}\underline{59.05}
& \textbf{36.60} & 28.80 & \underline{21.60} & \underline{32.60}
& \cellcolor{black!12}29.90
& \underline{19.80} & 9.80 & 2.40 & \underline{15.00}
& \cellcolor{black!12}11.75 \\

\bottomrule
\end{tabularx}
\end{table*}
